Learning Complex Teamwork Tasks Using a Given Sub-task Decomposition

Training a team to complete a complex task via multi-agent reinforcement learning can be difficult due to challenges such as policy search in a large joint policy space, and non-stationarity caused by mutually adapting agents. To facilitate efficient learning of complex multi-agent tasks, we propose an approach which uses an expert-provided decomposition of a task into simpler multi-agent sub-tasks. In each sub-task, a subset of the entire team is trained to acquire sub-task-specific policies. The sub-teams are then merged and transferred to the target task, where their policies are collectively fine-tuned to solve the more complex target task. We show empirically that such approaches can greatly reduce the number of timesteps required to solve a complex target task relative to training from-scratch. However, we also identify and investigate two problems with naive implementations of approaches based on sub-task decomposition, and propose a simple and scalable method to address these problems which augments existing actor-critic algorithms. We demonstrate the empirical benefits of our proposed method, enabling sub-task decomposition approaches to be deployed in diverse multi-agent tasks.

==> custom/convenience.tex <==
\newcommand{\tss}{\textsubscript}
\newcommand{\TSS}{\textsuperscript}

\newcommand{\BaselineFromScratch}{\textbf{from-scratch}}
\newcommand{\BaselinePreSkilled}{\textbf{pre-skilled}}
\newcommand{\BaselinePreSkilledBP}{\textbf{pre-skilled (BP)}}
\newcommand{\BaselinePreSkilledNoBP}{\textbf{pre-skilled (no-BP)}}
\newcommand{\BaselineMEDoE}{\textbf{\acs{MEDoE}}}
\newcommand{\BaselineMEDoEHC}{\textbf{\acs{MEDoE} (Expert)}}
\newcommand{\BaselineMEDoEMLP}{\textbf{\acs{MEDoE} (\acs{MLP})}}
\newcommand{\BaselineMEDoENoBP}{\textbf{\acs{MEDoE} (Expert, no-BP)}}

\newcommand{\BaselineMEDoENoClip}{\textbf{\acs{MEDoE} (no clip boost)}}
\newcommand{\BaselineMEDoENoEnt}{\textbf{\acs{MEDoE} (no ent. boost)}}
\newcommand{\BaselineMEDoENoKL}{\textbf{\acs{MEDoE} (no KL boost)}}
\newcommand{\BaselineMEDoENoTemp}{\textbf{\acs{MEDoE} (no temp boost)}}

